White-box Fuzzing RPC-based APIs with EvoMaster: An Industrial Case Study

Remote Procedure Call (RPC) is a communication protocol to support client-server interactions among services over a network. RPC is widely applied in industry for building large-scale distributed systems, such as Microservices. Modern RPC frameworks include for example Thrift, gRPC, SOFARPC and Dubbo. Testing such systems is very challenging, due to the complexity of distributed systems and various RPC frameworks the system could employ. To the best of our knowledge, there does not exist any tool or solution that could enable automated testing of modern RPC-based services. To fill this gap, in this paper we propose the first approach in the literature, together with an open-source tool, for white-box fuzzing modern RPC-based APIs with search. To assess our novel approach, we conducted an empirical study with two artificial and four industrial APIs selected by our industrial partner. The tool has been integrated into a real industrial pipeline, and could be applied to real industrial development process for fuzzing RPC-based APIs. To further demonstrate its effectiveness and application in industrial settings, we also report results of employing our tool for fuzzing another 50 industrial APIs autonomously conducted by our industrial partner in their testing processes. Results show that our novel approach is capable of enabling automated test case generation for industrial RPC-based APIs (i.e., two artificial and 54 industrial). We also compared with a simple grey-box technique and existing manually written tests. Our white-box solution achieves significant improvements on code coverage. Regarding fault detection, by conducting a careful review with our industrial partner of the tests generated by our novel approach in the selected four industrial APIs, a total of 41 real faults were identified, which have now been fixed. Another 8,377 detected faults are currently under investigation.

==> tables/comparison-exisiting-class.tex <==
\begin{tabular}{l rrrr}
	\toprule 
	& RPC-EVO (\%)  & Ex.(\%) & Total (\%) & Uncover.(\%) \\
	\textit{SUT} & [$W$, $B$] & $E$ & [$W \cup E$, $B\cup E$] & [$W$-$E$, $B$-$E$] \\
	\midrule
	\csA & [\underline{59.82}, 74.11] & 59.82 & [67.86, 75.89] & [8.04, 1.79] \\
	\csB & [65.52, 67.82] & 48.85 & [65.52, 67.82] & [0.00, 0.00] \\
	\csC & [44.07, 48.99] & 27.74 & [44.07, 48.99] & [0.00, 0.00] \\
	\csD & [42.48, 43.85] & 40.17 & [44.58, 45.43] & [2.10, 1.58] \\
	\midrule
\textit{Avg.} & [52.97, 58.69] & 44.15 & [55.51, 59.53] & [2.53, 0.84] \\
	\bottomrule 
\end{tabular}

==> tables/comparison-exisiting-method.tex <==
\begin{tabular}{l rrrr}
	\toprule 
	& RPC-EVO (\%)  & Ex.(\%) & Total (\%) & Uncover.(\%) \\
	\textit{SUT} & [$W$, $B$] & $E$ & [$W \cup E$, $B\cup E$] & [$W$-$E$, $B$-$E$] \\
	\midrule
	\csA & [24.19, 28.91] & 15.22 & [24.32, 29.40] & [0.12, 0.50] \\
	\csB & [24.36, 25.00] & 13.86 & [24.36, 25.00] & [0.00, 0.00] \\
	\csC & [20.58, 23.82] & 7.43 & [20.65, 23.86] & [0.07, 0.04] \\
	\csD & [\phantom{0}8.28, \phantom{0}9.20] & 7.44 & [\phantom{0}9.61, 10.37] & [1.34, 1.16] \\
	\midrule
	\textit{Avg.} & [19.35, 21.73] & 10.99 & [19.73, 22.16] & [0.38, 0.42] \\
	\bottomrule 
\end{tabular}
